Semi-Lagrangian Subgrid Reconstruction for Advection-Dominant Multiscale Problems

We introduce a new framework of numerical multiscale methods for advection-dominated problems motivated by climate sciences. Current numerical multiscale methods (MsFEM) work well on stationary elliptic problems but have difficulties when the model involves dominant lower order terms. Our idea to overcome the assocociated difficulties is a semi-Lagrangian based reconstruction of subgrid variablity into a multiscale basis by solving many local inverse problems. Globally the method looks like a Eulerian method with multiscale stabilized basis. We show example runs in one and two dimensions and a comparison to standard methods to support our ideas and discuss possible extensions to other types of Galerkin methods, higher dimensions and nonlinear problems.

==> fig-2d_multiscale_mesh.tex <==
\begin{wrapfigure}{l}{0.4\textwidth}
  \vspace{-10pt}
  \begin{center}
    \includegraphics[width=0.39\textwidth]{fig-2d_multiscale_mesh.pdf}
  \end{center}
  \vspace{0pt}
  \caption{Global coarse mesh and local fine mesh in 2D.}
  \vspace{-10pt}
  \label{fig-2d_multiscale_mesh}
\end{wrapfigure}
